EMIXER: End-to-end Multimodal X-ray Generation via Self-supervision

Deep generative models have enabled the automated synthesis of high-quality data for diverse applications. However, the most effective generative models are specialized to data from a single domain (e.g., images or text). Real-world applications such as healthcare require multi-modal data from multiple domains (e.g., both images and corresponding text), which are difficult to acquire due to limited availability and privacy concerns and are much harder to synthesize. To tackle this joint synthesis challenge, we propose an End-to-end MultImodal X-ray genERative model (EMIXER) for jointly synthesizing x-ray images and corresponding free-text reports, all conditional on diagnosis labels. EMIXER is an conditional generative adversarial model by 1) generating an image based on a label, 2) encoding the image to a hidden embedding, 3) producing the corresponding text via a hierarchical decoder from the image embedding, and 4) a joint discriminator for assessing both the image and the corresponding text. EMIXER also enables self-supervision to leverage vast amount of unlabeled data. Extensive experiments with real X-ray reports data illustrate how data augmentation using synthesized multimodal samples can improve the performance of a variety of supervised tasks including COVID-19 X-ray classification with very limited samples. The quality of generated images and reports are also confirmed by radiologists. We quantitatively show that EMIXER generated synthetic datasets can augment X-ray image classification, report generation models to achieve 5.94% and 6.9% improvement on models trained only on real data samples. Taken together, our results highlight the promise of state of generative models to advance clinical machine learning.

==> Tables/comparison.tex <==
\begin{table}[!h]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{lrrr}
\toprule
\textbf{Method} & {\begin{tabular}[r]{@{}r@{}}\textbf{Macro-F1}\\ Benign / Noisy\end{tabular}} & \textbf{\begin{tabular}[r]{@{}r@{}}Params\\ ($\times 10^6$)\end{tabular}} & \textbf{\begin{tabular}[r]{@{}r@{}}Flops\\ ($\times 10^9$)\end{tabular}} \\ \hline
Sors & - & 2.26 & 1.45 \\
Biswal & - & 9.62 & 26.61 \\
Deep Residual & - & 18.62 & 6.49 \\
\method(sors) & - & - & - \\
\method(Biswal) & - & - & - \\
\method(Scott) & - & - & - \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Benchmark of recent SOTA \scott{what is SOTA?} models on the benign and gaussian noise corrupted sleep-EDF dataset.}
\label{tab:model_comparrson}
\end{table}

==> Tables/confusion-matrix.tex <==



\begin{table*}[t]
    \setlength{\tabcolsep}{9.2pt}
    % \small
    \centering
     \begin{tabular}{lcccccccc}  %lrrrrrrrr
     \toprule
     & \multicolumn{5}{c}{{\textbf{Predicted}}} & \multicolumn{3}{c}{{\textbf{Per-class Metrics}}} \\
     \cmidrule(l){2-6}\cmidrule(l){7-9}
     & W & N1  & N2  & N3 & REM & PR  & RE & F1  \\ 
    %  [0.5ex] 
     \midrule
    W & \textbf{1825 / 2345} & 26 / 71 & 58 / 44 & 0 / 1 & 127 / 136 & 0.98 / 0.93 & 0.70 / 0.90 & 0.82 / 0.91  \\
    N1 & 15 / 98 & \textbf{125 / 172} & 101 / 70 & 0 / 0 & 151 / 52 & 0.45 / 0.42 & 0.32 / 0.44 & 0.37 / 0.43  \\
    N2 & 16 / 54 & 22 / 85 & \textbf{3820 / 3812} & 161 / 94 & 89 / 63 & 0.83 / 0.85 & 0.93 / 0.93 & 0.88 / 0.89  \\
    N3 & 1 / 1 & 0 / 0 & 296 / 410 & \textbf{1128 / 1014} & 0 / 0 & 0.87 / 0.91 & 0.79 / 0.71 & 0.83 / 0.80  \\
    REM & 5 / 36 & 16 / 79 & 240 / 128 & 1 / 1 & \textbf{1342 / 1360} & 0.64 / 0.84 & 0.84 / 0.85 & 0.72 / 0.85  \\
    \bottomrule
    \end{tabular}
    \caption{Confusion matrix evaluating the performance of the \method-Sors$_C$(A+S) and benign trained Sors$_C$ model on the SHHS test dataset containing no noise. Our \method{} trained model is on the left, baseline right.}
    \label{tab:confusion-benign}
\end{table*}


\begin{table*}[t]
    % \setlength{\tabcolsep}{10pt}
    % \small
    \setlength{\tabcolsep}{10pt}
    \centering
     \begin{tabular}{lrrrrrrrr} 
     \toprule
     & \multicolumn{5}{c}{{\textbf{Predicted}}} & \multicolumn{3}{c}{{\textbf{Per-class Metrics}}} \\
     \cmidrule(l){2-6}\cmidrule(l){7-9}
     & W & N1  & N2  & N3 & REM & PR  & RE & F1  \\ 
    %  [0.5ex] 
     \midrule
    W & \textbf{2386 / 2564} & 26 / 4 & 58 / 29 & 0 & 127 / 0 & 0.93 / 0.63 & 0.92 / 0.99 & 0.92 / 0.77  \\
    N1 & 91 / 287 & \textbf{112 / 44} & 57 / 59 & 0 / 0 & 133 / 2 & 0.54 / 0.16 & 0.29 / 0.11 & 0.37 / 0.13  \\
    N2 & 43 / 357 & 44 / 42 & \textbf{3614 / 3686} & 165 / 22 & 242 / 1 & 0.89 / 0.70 & 0.88 / 0.90 & 0.89 / 0.79  \\
    N3 & 2 / 47 & 0 / 0 & 261 / 1003 & \textbf{1162 / 375} & 0 / 0 & 0.88 / 0.94 & 0.82 / 0.26 & 0.84 / 0.41  \\
    REM & 47 / 830 & 24 / 192 & 55 / 483 & 1 / 0 & \textbf{1477 / 99} & 0.75 / 0.97 & 0.92 / 0.06 & 0.82 / 0.12  \\
    \bottomrule
    \end{tabular}
    \caption{Confusion matrix evaluating the performance of the REST-Sors$_C$(A+S) model on the SHHS test dataset containing Gaussian noise at the medium level. Our \method{} trained model is on the left, baseline right.}
    \label{tab:confusion-guassian}
\end{table*}




==> Tables/datasets.tex <==


\begin{table}[b]
    % \setlength{\tabcolsep}{10pt}
    \small
    \centering
     \begin{tabular}{lrrrrrr} 
     \toprule
     \textbf{Dataset} & \textbf{W} & \textbf{N1}  & \textbf{N2}  & \textbf{N3}(N4) & \textbf{REM} & \textbf{Total}  \\ 
    %  [0.5ex] 
     \midrule
     Sleep-EDF & 8,168 & 2,804 & 17,799 & 5,703 & 7,717 & 42,191  \\
     SHHS & 28,854 & 3,377 & 41,246 & 13,409 & 13,179 & 100,065  \\
    \bottomrule
    \end{tabular}
    \caption{Dataset summary outlining the number of 30 second EEG recordings belonging to each sleep stage class.}
    \label{tab:dataset-summary}
\end{table}

==> Tables/efficiency_table.tex <==
\begin{table}[t!]
    \setlength{\tabcolsep}{14pt}
    \centering
     \begin{tabular}{c|lrr} 
     \toprule
     \textbf{Data} & \textbf{Model} & \textbf{Size} (KB)  & \textbf{MFlops} \\ 
    %  [0.5ex] 
     \midrule
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Sleep-EDF}}}
     & Sors~\cite{sors2018convolutional} & 8,896 & 1451 \\
     & Liu~\cite{liu2017learning} & \textbf{440} & 127 \\
     & Blanco~\cite{blanco1997applying} & 440 & 127 \\
     & Ford~\cite{Ford2019} & 448 & 144 \\ 
     & \method(A) & 464 & 98 \\ 
     & \method(A+S) & 449 & \textbf{94} \\ 
     
      \midrule%\cdashlinelr{1-6} 
     
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{SHHS}}}
     & Sors~\cite{sors2018convolutional} & 8,996 & 1815 \\
     & Liu~\cite{liu2017learning} & \textbf{464} & 211 \\
     & Blanco~\cite{blanco1997applying} & 464 & 211 \\
     & Ford~\cite{Ford2019} & 478 & 170 \\ 
     & \method(A) & 476 & 160 \\ 
     & \method(A+S) & 496 & \textbf{142} \\ 
    \bottomrule
    \end{tabular}
    \captionof{table}{
        Comparison on model size and the FLOPS required to score a single night of EEG recordings. \method{} models are significantly smaller and comparable in size/compute to baselines. 
    }
    \label{tab:efficiency}
    \vspace{-0.3cm}
\end{table}
  


 


==> Tables/gaussian-search.tex <==


\begin{table}[!t]
    \setlength{\tabcolsep}{5.7pt}
    \centering
     \begin{tabular}{crrrrrr} 
     \toprule
     & & & \multicolumn{3}{c}{{\textbf{Guassian F1}}} & \\
    \cmidrule(l){4-6} 
     
    & \textbf{$c_g$} &  \textbf{Benign F1} & \textbf{Low} & \textbf{Med} & \textbf{High} & \textbf{Average F1} \\
    \midrule
    
    \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{EDF}}}
    & 0.1 & 0.75 & 0.76 & 0.7 & 0.5 & 0.68 \\
    &  0.2 & 0.7 & 0.72 & 0.75 & 0.64 & \textbf{0.70} \\
    & 0.3 & 0.67 & 0.68 & 0.71 & 0.75 & 0.7025 \\
     
    \midrule

    \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{SHHS}}}
    & 0.1 & 0.69 & 0.74 & 0.45 & 0.21 & 0.52 \\
    & 0.2 & 0.68 & 0.69 & 0.68 & 0.43 & \textbf{0.62} \\
    & 0.3 & 0.55 & 0.57 & 0.65 & 0.74 & 0.63 \\
    \bottomrule
    \end{tabular}
    \caption{Line search results for identifying optimal $c_g$ on Sleep-EDF and SHHS datasets. Macro-F1 is abbreviated F1 in table; average macro-F1 is the mean of all macro-F1 scores.
    We select $c_g$=0.2 for both datasets as it represents a good trade-off between benign and Gaussian macro-F1.
    }
    \label{tab:line-search-gaussian}
\end{table}

==> Tables/lambda-search.tex <==
\begin{table}[!h]
\setlength{\tabcolsep}{5.3pt}
    \centering
     \begin{tabular}{rrrrrrr} 
     \toprule
     & & & \multicolumn{3}{c}{{\textbf{Adversarial F1}}} & \\
    \cmidrule(l){4-6} 
     
     \textbf{$\lambda_o$} & \textbf{$\lambda_g$} & \textbf{Benign F1} & \textbf{Low} & \textbf{Med} & \textbf{High} & \textbf{Avg. F1} \\
     \midrule
     
    0.001 & 1E-04 & 0.73 & 0.66 & 0.65 & 0.61 & 0.66 \\
    0.003 & 1E-04 & 0.72 & 0.64 & 0.63 & 0.59 & 0.65 \\
    0.005 &	1E-04 & 0.72 & 0.65 & 0.64 & 0.62 & 0.66 \\
    0.001 &	1E-05 &	0.73 & 0.66 & 0.65 & 0.62 & 0.67 \\
    \rowcolor{lightgray} 
    0.003 & 1E-05 & 0.73 & 0.67 & 0.66 & 0.62 & \textbf{0.67} \\
    0.005 &	1E-05 & 0.73 & 0.64 & 0.64 & 0.62 & 0.66 \\
    \bottomrule
    \end{tabular}
    \captionof{table}{Grid search results for $\lambda_o$ and $\lambda_g$ on Sleep-EDF dataset. 
    Macro-F1 is abbreviated as F1 in table; average macro-F1 is the mean of all macro-F1 scores.
    We select $\lambda_o$ and $\lambda_g$ with highest average macro-F1 score.
    }
    \label{tab:grid-search-lambdas}
\end{table}

==> Tables/noise_table.tex <==



\begin{table*}[t!]
\setlength{\tabcolsep}{2.5pt}
\centering

 \begin{tabular}{clcrrrrrrrrrr }
 \toprule
 & & & & \multicolumn{3}{c}{\textbf{Adversarial}} & \multicolumn{3}{c}{\textbf{Gaussian}} & \multicolumn{3}{c}{\textbf{Shot}} \\
%  & & & \textbf{Adversarial} & \textbf{Gaussian} & \textbf{Shot} \\ 
\cmidrule(l){5-7} \cmidrule(l){8-10} \cmidrule(l){11-13} 
 
 \textbf{Data} & \textbf{Method}  & \textbf{Compress} & \textbf{No noise} & Low & Med & High & Low & Med & High & Low & Med & High \\ 
%  [0.3ex] 
 \midrule
 \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Sleep-EDF}}}
 
 \vspace{2mm} & Sors \cite{sors2018convolutional} & \xmark & 0.67 \s{0.02} & 0.57 \s{0.02} & 0.51 \s{0.04} & 0.19 \s{0.06} & 0.66 \s{0.03} & 0.60 \s{0.03} & 0.39 \s{0.08} & 0.58 \s{0.04} & 0.42 \s{0.08} & 0.11 \s{0.03} \\ 
 
 & Liu \cite{liu2017learning} & \cmark & \textbf{0.69} \s{0.02} & 0.52 \s{0.07} & 0.41 \s{0.07} & 0.09 \s{0.02} & 0.67 \s{0.02} & 0.53 \s{0.02} & 0.28 \s{0.04} & 0.52 \s{0.03} & 0.31 \s{0.04} & 0.06 \s{0.01} \\ 
 & Blanco \cite{blanco1997applying} & \cmark & 0.68 \s{0.01} & 0.51 \s{0.06} & 0.40 \s{0.06} & 0.09 \s{0.02} & 0.65 \s{0.02} & 0.54 \s{0.04} & 0.31 \s{0.10} & 0.53 \s{0.04} & 0.34 \s{0.09} & 0.08 \s{0.02} \\ 
 \vspace{2mm} & Ford \cite{Ford2019} & \cmark & 0.64 \s{0.01} & 0.59 \s{0.01} & 0.60 \s{0.02} & 0.31 \s{0.08} & 0.65 \s{0.01} & 0.67 \s{0.02} & 0.57 \s{0.03} & 0.67 \s{0.02} & 0.60 \s{0.02} & 0.10 \s{0.01} \\ 

 & \method(A) & \cmark & 0.66 \s{0.02} & 0.64 \s{0.02} & 0.64 \s{0.02} & 0.61 \s{0.02} & 0.66 \s{0.02} & 0.67 \s{0.01} & 0.66 \s{0.01} & 0.67 \s{0.01} & 0.66 \s{0.01} & \textbf{0.42} \s{0.06} \\ 
 & \method(A+S) & \cmark & \textbf{0.69} \s{0.01} & \textbf{0.67} \s{0.02} & \textbf{0.66} \s{0.01} & \textbf{0.61} \s{0.03} & \textbf{0.69} \s{0.01} & \textbf{0.68} \s{0.01} & \textbf{0.67} \s{0.02} & \textbf{0.68} \s{0.01} & \textbf{0.67} \s{0.02} & \textbf{0.42} \s{0.08} \\ 
 
 \midrule
 
 \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{SHHS}}}
 \vspace{2mm} & Sors \cite{sors2018convolutional} & \xmark & \textbf{0.78} \s{0.01} & 0.62 \s{0.03} & 0.46 \s{0.03} & 0.33 \s{0.00} & 0.64 \s{0.03} & 0.43 \s{0.02} & 0.35 \s{0.04} & 0.69 \s{0.02} & 0.59 \s{0.03} & 0.45 \s{0.01} \\ 
 
 & Liu \cite{liu2017learning} & \cmark & 0.77 \s{0.01} & 0.61 \s{0.02} & 0.49 \s{0.04} & 0.34 \s{0.03} & 0.66 \s{0.05} & 0.45 \s{0.05} & 0.34 \s{0.04} & 0.70 \s{0.04} & 0.62 \s{0.04} & 0.47 \s{0.05} \\ 
 & Blanco \cite{blanco1997applying} & \cmark & 0.77 \s{0.01} & 0.60 \s{0.03} & 0.47 \s{0.04} & 0.33 \s{0.02} & 0.64 \s{0.07} & 0.43 \s{0.05} & 0.34 \s{0.04} & 0.67 \s{0.06} & 0.59 \s{0.05} & 0.46 \s{0.04} \\ 
 \vspace{2mm}& Ford \cite{Ford2019} & \cmark & 0.62 \s{0.02} & 0.59 \s{0.01} & 0.62 \s{0.00} & 0.59 \s{0.05} & 0.66 \s{0.00} & 0.75 \s{0.04} & 0.47 \s{0.10} & 0.65 \s{0.00} & 0.68 \s{0.01} & 0.74 \s{0.04} \\ 

 & \method(A) & \cmark & 0.70 \s{0.01} & 0.68 \s{0.00} & 0.70 \s{0.01} & 0.67 \s{0.01} & 0.72 \s{0.01} & 0.76 \s{0.01} & 0.58 \s{0.03} & 0.72 \s{0.01} & 0.74 \s{0.01} & 0.76 \s{0.01}  \\ 
 & \method(A+S) & \cmark & 0.72 \s{0.01} & \textbf{0.69} \s{0.01} & \textbf{0.70} \s{0.01} & \textbf{0.69} \s{0.02} & \textbf{0.74} \s{0.01} & \textbf{0.77} \s{0.01} & \textbf{0.62} \s{0.03} & \textbf{0.73} \s{0.01} & \textbf{0.75} \s{0.01} & \textbf{0.78} \s{0.00} \\ 
 
\bottomrule
\end{tabular}
\caption{
Meta Analysis: Comparison of macro-F1 scores achieved by each model. The models are evaluated on Sleep-EDF and SHHS datasets with three types and strengths of noise corruption. 
We bold the compressed model with the best performance (averaged over 3 runs) and report the standard deviation of each model next to the macro-F1 score. 
\method{} performs better in \textit{all} noise test measurements. 
}
\label{tab:noise-robustness}
\end{table*}




==> mathdef.tex <==

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}
% helpful math macros
\newcommand{\xseq}{x_{n,1:\text{T}_n}}
\newcommand{\eye}{\mathbf{I}}
%\newcommand{\real}[1]{\mathbb{R}^{#1}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\data}{\mathcal{D}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\KL}[2]{\text{KL}(#1 \text{ } || \text{ }#2)}
\newcommand{\ent}[1]{\mathbb{H}({#1})}
\newcommand{\elbo}{\mathcal{L}}
\newcommand{\squash}{\xi}
\newcommand{\grad}[1]{\nabla_{#1}}
\newcommand{\es}{s}
\newcommand{\rpm}{\raisebox{.2ex}{$\scriptstyle\pm$}}

% method's name definition
%\newcommand{\mname}{\texttt{EHRVAE}\xspace}

% \newcommand{\js1}[1]{{\color{blue} [J: #1]}}
%from Vagelis:
\newcommand{\reminder}[1]{{\textsf{\textcolor{red}{[#1]}}}}

